A Systematic Search for Reddest Far-infrared and Sub-millimeter Galaxies: revealing dust-embedded starbursts at high redshifts

We present the results of our systematic search for the reddest far-infrared (FIR) and submillimeter (sub-mm) galaxies using the data from the Herschel Multi-tiered Extragalactic Survey (HerMES) and the SCUBA2 Cosmological Legacy Survey (S2CLS). The red FIR galaxies are "500~$\mu$m risers," whose spectral energy distributions increase with wavelength across the three FIR passbands of the Spectral and Photometric Imaging REceiver (SPIRE) of Herschel. Within 106.5 deg$^2$ of the HerMES fields, we have selected 629 500 $\mu$m risers. The red sub-mm galaxies are "SPIRE dropouts," which are prominent detections in the S2CLS 850 $\mu$m data but are extremely weak or invisible in the SPIRE bands. Within the 2.98 deg$^2$ common area of HerMES and S2CLS, we have selected 95 such objects. These very red sources could be dusty starbursts at high redshifts ($z\gtrsim 4$-6) because the peak of their cold-dust emission heated by star formation is shifted to the reddest FIR/sub-mm bands. The surface density of 500 $\mu$m risers is $\sim$8.2 deg$^{-2}$ at the $\geq 20$ mJy level in 500 $\mu$m, while that of SPIRE dropouts is $\sim$19.3 deg$^{-2}$ at the $\geq 5$ mJy level in 850 $\mu$m. Both type of objects could span a wide range of redshifts, however. Using deep radio data in these fields to further select the ones likely at the highest redshifts, we find that the surface density of $z>6$ candidates is 5.5 deg$^{-2}$ among 500 $\mu$m risers and is 0.8-13.6 deg$^{-2}$ among SPIRE dropouts. If this is correct, the dust-embedded star formation processes in such objects could contribute comparably as Lyman-break galaxies to the global SFR density at $z>6$.

==> emulateapj_look_and_feel.tex <==
% vim:ft=tex:
%
\makeatletter
%%%%%%%% The following code is taken from size10.clo; it fixes
%%%%%%%% aastex's definition of type sizes
\renewcommand\normalsize{%
   \@setfontsize\normalsize\@xpt{10.56}
   \abovedisplayskip 2.2mm \@plus2\p@ \@minus1\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 2.2mm \@plus2\p@ \@minus1\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\renewcommand\small{%
   \@setfontsize\small\@ixpt{9.68}%
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 4\p@ \@plus2\p@ \@minus2\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\renewcommand\footnotesize{%
   \@setfontsize\footnotesize\@viiipt{8.36}%
   \abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus\p@
   \belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 3\p@ \@plus\p@ \@minus\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\renewcommand\scriptsize{\@setfontsize\scriptsize\@viipt\@viiipt}
\renewcommand\tiny{\@setfontsize\tiny\@vpt\@vipt}
\renewcommand\large{\@setfontsize\large\@xiipt{14}}
\renewcommand\Large{\@setfontsize\Large\@xivpt{18}}
\renewcommand\LARGE{\@setfontsize\LARGE\@xviipt{22}}
\renewcommand\huge{\@setfontsize\huge\@xxpt{25}}
\renewcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}
\setlength\smallskipamount{3\p@ \@plus 1\p@ \@minus 1\p@}
\setlength\medskipamount{6\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\bigskipamount{12\p@ \@plus 4\p@ \@minus 4\p@}
\setlength\headheight{12\p@}
\def\@listi{\leftmargin\leftmargini
            \parsep 4\p@ \@plus2\p@ \@minus\p@
            \topsep 8\p@ \@plus2\p@ \@minus4\p@
            \itemsep4\p@ \@plus2\p@ \@minus\p@}
\let\@listI\@listi
\@listi
\def\@listii {\leftmargin\leftmarginii
              \labelwidth\leftmarginii
              \advance\labelwidth-\labelsep
              \topsep    4\p@ \@plus2\p@ \@minus\p@
              \parsep    2\p@ \@plus\p@  \@minus\p@
              \itemsep   \parsep}
\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep
              \topsep    2\p@ \@plus\p@\@minus\p@
              \parsep    \z@
              \partopsep \p@ \@plus\z@ \@minus\p@
              \itemsep   \topsep}
\def\@listiv {\leftmargin\leftmarginiv
              \labelwidth\leftmarginiv
              \advance\labelwidth-\labelsep}
\def\@listv  {\leftmargin\leftmarginv
              \labelwidth\leftmarginv
              \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
              \labelwidth\leftmarginvi
              \advance\labelwidth-\labelsep}
% no bf title
\def\frontmatter@title@format{
%% No exception for rnaas, May, 2019
%\ifrnaas
%\large\scshape\centering
%\else
\normalsize
%% added Mar 2019
\centering
%\fi
 }
\makeatother
% all cap title
\usepackage{letltxmacro}
\LetLtxMacro{\aastextitle}{\title}
\renewcommand{\title}[1]{\uppercase{\aastextitle{#1}}}

